Reasoning with Probabilities: Relating Weighted Model Counting and Probabilistic Model Checking

Weighted model counting (WMC) and probabilistic model checking (PMC) are two well- established frameworks that are independently developed, the former for probabilistic inference, the latter traditionally for probabilistic verification, though recently also applied to inference. The formal relationship between the two frameworks, however, remains largely unexplored. In this paper, we lay the foundations for how they relate: we present (1) a mapping from cycle- free parametric Markov chains (pMCs) to arithmetic circuits (ACs), enabling the reduction of reachability probability computations in such pMCs to a weighted model counting problem on the corresponding ACs, and (2) a mapping from a subclass of arithmetic circuits -- with probabilistic semantics -- back to parametric Markov chains. We propose a detailed correspondence between the entities of WMC and PMC, and discuss how our mappings enable transferring optimization techniques such as bisimulation minimization across the frameworks.

==> bisimulation.tex <==
%\enlargethispage{2\baselineskip}

In this section, we overview the formal definitions related to Bisimulation minimization. 
\begin{definition} 
\label{def-bisim-rel}
Let $\mathcal{M} = (S, s_0, X, \mbox{Lits}, L, {P})$ be a (parametric) Markov chain. A {probabilistic bisimulation} is an \emph{equivalence relation} $\mathcal{R}$ on $S$ such that for all pairs $(s_1,s_2) \in \mathcal{R}$,
\begin{itemize}
\item $L(s_1) = L(s_2)$,
\item $\mathcal{P}(s_1, T) = \mathcal{P}(s_2, T)$, for each equivalence class $T \in S |_{\mathcal{R}}$,
where $\mathcal{P}(s, T) = \sum\limits_{t \in T} \mathcal{P}(s, t)$.
\end{itemize}
The states $s_1$ and $s_2$ are {bisimulation equivalent} (or bisimilar), denoted by $s_1 \sim_{\mathcal{R}} s_2$ iff there is a bisimulation relation $\mathcal{R}$ on $\mathcal{M}$ such that $(s_1, s_2) \in \mathcal{R}$.
\end{definition}


\par \noindent Intuitively speaking, The bisimilar states (i) have the same labels, and (ii) move to the same equivalent classes with the same (accumulative) probabilities. 
\begin{example} 
\label{ex-bisim-def}
Consider the MC $\mathcal{M}$ in Fig.~\ref{fig:chap-prel-bisim}(a) with $\mbox{Lits} = \{r, \neg r\}$ and $L(s_7) = L(s_9) = r$, $L(s_8) = L(s_{10}) = \neg r$, and $L(s_i) = \emptyset$ for all other states. The states $s_{11}$ and $s_{12}$ are bisimulation equivalent:  $L(s_{11}) = L(s_{12}) = \emptyset$ and $\mathcal{P}(s_{11}, T) = \mathcal{P}(s_{12}, T) = 1$ for the single successive class $T$ (self). We denote them as the class $[s_{11}]_{\sim
}$ or $[s_{12}]_{\sim
}$. The states $s_7$ and $s_9$ are also bisimilar, denoted by $[s_7]_{\sim
}$ or $[s_9]_{\sim
}$: (i) their labels are the same $L(s_{7}) = L(s_{9}) = R$ and (ii) their accumulative transition probability to their successive class is identical; we have $\mathcal{P}(s_7, [s_{11}] ) = 0.01 + 0.99 = \mathcal{P}(s_9, [s_{11}] ) = 0.1 + 0.9 = 1$. We similarly have $s_8 \sim_{\mathcal{R}} s_{10}$, $ s_{3} \sim_{\mathcal{R}} s_4$, and $s_{5} \sim_{\mathcal{R}} s_6$.
\end{example}
\par \noindent Informally speaking, the \emph{quotient Markov chain} of a MC is a MC in which the bisimilar states are merged. Below, we review the defintion followed by an example (see Figure \ref{fig:chap-prel-bisim}). We then emphasize on an interesting characteristic of the \emph{quotient MC} on preserving the reachability probabilities. 
\begin{definition} 
\label{def-bisim-quo}
Let $\mathcal{M} = (S, s_0, \mbox{Lits}, L, P)$ be a Markov chain. The \emph{quotient Markov chain} of $\M$ is $\mathcal{M}  |_{\mathcal{R}} = (S |_{\mathcal{R}}, \mathcal{P}', s_0, \mbox{Lits}, L')$, where $\mathcal{P}'([s]_{
\mathcal{R}}, [t]_{\mathcal{R}}) = \mathcal{P}(s, [t]_{\mathcal{R}})$ and $L'([s]_{\mathcal{R}}) = L(s)$.
\end{definition}
\par \noindent The state space of the quotient Markov chain is the set of equivalence classes under the relation $\mathcal{R}$. The transition probability from the equivalence class $[s]_{\mathcal{R}}$ to the equivalence class $[t]_{\mathcal{R}}$ is given by  $\mathcal{P}(s, [t]_{\mathcal{R}})$. Any member of the equivalence class $[s]_{\mathcal{R}}$ can be an alternative to $s$ as $\mathcal{P}(s, T) = \mathcal{P}(s', T)$ for all classes $T$ and all $s' \sim_{\mathcal{R}} s$ by definition.


\input{images/bisim-example}

\begin{example} Figure \ref{fig:chap-prel-bisim}(b) shows the \emph{quotient Markov chain} for the MC in Fig.~\ref{fig:chap-prel-bisim}, where the bisimilar states are merged. We showed in Example \ref{ex-bisim-def} that $s_3 \sim_{\mathcal{R}} s_4$, $s_5 \sim_{\mathcal{R}} s_6$, $s_7 \sim_{\mathcal{R}} s_9$, $s_8 \sim_{\mathcal{R}} s_{10}$, and $s_{11} \sim_{\mathcal{R}} s_{12}$. 
\end{example}

\par \noindent The \emph{quotient Markov chain}  $\mathcal{M} | _{\mathcal{R}}$ for the MC preserves the reachability probabilities in $\mathcal{M}$ with respect to the literals $\mbox{Lits}$, that is for each $lits \subseteq \mbox{Lits}$, 
\begin{align*}
\Pr_{\mathcal{M} |_{\mathcal{R}}} (\lozenge lits) = \Pr_{\mathcal{M}} (\lozenge lits).
\end{align*}

\begin{example}
For the MC in Fig. \ref{fig:chap-prel-bisim} (a) and its quotient Markov chain in Fig. \ref{fig:chap-prel-bisim} (b), we have $\Pr_{\mathcal{M}} (\lozenge \, r) = \Pr_{\mathcal{M} |_{\mathcal{R}}} (\lozenge \, r) = 0.5$.
\end{example}

\par \noindent We consider \emph{bisimulation equivalence} with respect to a given reachability query $\Pr_{\M}(\lozenge G)$. Let $\mbox{Lits}_G$ denote the set of literals that appear in $G$. Let $L_{G}(s)  = L(s) \cap \mbox{Lits}$ denote the $G$-relavant labeling for state $s$. If $s$'s label appears in the query, $L_G(s) = L(s)$, otherwise $L_G(s) = \emptyset$.  To consider \emph{bisimulation equivelance} for the MC $\mathcal{M}$ regarding the reachability query $\Pr_{\M}(\lozenge G)$, it suffices to replace $L$ by $L_{G}$ in Def.\ref{def-bisim-rel} and \ref{def-bisim-quo}.

